DA4AD: End-to-End Deep Attention-based Visual Localization for Autonomous Driving

We present a visual localization framework based on novel deep attention aware features for autonomous driving that achieves centimeter level localization accuracy. Conventional approaches to the visual localization problem rely on handcrafted features or human-made objects on the road. They are known to be either prone to unstable matching caused by severe appearance or lighting changes, or too scarce to deliver constant and robust localization results in challenging scenarios. In this work, we seek to exploit the deep attention mechanism to search for salient, distinctive and stable features that are good for long-term matching in the scene through a novel end-to-end deep neural network. Furthermore, our learned feature descriptors are demonstrated to be competent to establish robust matches and therefore successfully estimate the optimal camera poses with high precision. We comprehensively validate the effectiveness of our method using a freshly collected dataset with high-quality ground truth trajectories and hardware synchronization between sensors. Results demonstrate that our method achieves a competitive localization accuracy when compared to the LiDAR-based localization solutions under various challenging circumstances, leading to a potential low-cost localization solution for autonomous driving.

==> sources/loss.tex <==
\section{Loss Function}

In the inference stage, three weighted $L^3$-Net modules are connected in the order of FPN resolution from coarse to fine to predict the offset step by step. However, in the training stage, the three modules are independent of each other. Their input is the same predicted pose, and their outputs are independently too. Therefore, each module is treated independently, using the random poses generated from ground truth as the input, and desining the loss function based on the result of the module, so as to achieve adequate training for each module.

Our loss function includes three terms. The first one define the loss as squared $L$2 distance between the estimated offset $\hat{\Delta T} = (\hat{\Delta x}, \hat{\Delta y}, \hat{\Delta \psi})$ and the ground truth $\Delta T^* = (\Delta x^*, \Delta y^*, \Delta \psi^*)$. The estimated offset can be calculated by:

\begin{small}
	\begin{equation}
	\label{equ:predictedoffset}
	\hat{\Delta T} = (\sum_{i=1}^{n_x} P_i(\Delta x_i) \cdot \Delta x_i, \sum_{j=1}^{n_y} P_j(\Delta y_j) \cdot \Delta y_j, \sum_{k=1}^{n_\psi} P_k(\Delta \psi_k) \cdot \Delta \psi_k)
	\end{equation}
\end{small}
The loss function is defined as below:
\begin{small}
	\begin{equation} \label{equ:loss}
	Loss_1 = \alpha \cdot (\lVert \hat{\Delta x} - \Delta x^* \rVert^2 + \lVert \hat{\Delta y} - \Delta y^* \rVert^2) + \lVert \hat{\Delta \psi} - \Delta \psi^* \rVert^2,
	\end{equation}
\end{small}
where $\alpha$ is the balancing factor.

The second term of our loss function measures the similarity between deep features from online image and map. Under the projection of the ground truth pose, the corresponding 2D/3D keypoint pairs of online image and map should have the same or similar deep features. Therefore, the loss function is defined as below:

\begin{small}
	\begin{equation} \label{equ:loss2}
	Loss_2 = \sum_{i=0}^{K} \max(||F_i^M - F_i^I||^2-C, 0),
	\end{equation}
\end{small}
where $F_i^M$ and $F_i^M$ are descriptors of keypoints from online image and map, and $C$ is a constant, set to 1.

















